Seeing the Reasoning: How LLM Rationales Influence User Trust and Decision-Making in Factual Verification Tasks

Large Language Models (LLMs) increasingly show reasoning rationales alongside their answers, turning "reasoning" into a user-interface element. While step-by-step rationales are typically associated with model performance, how they influence users' trust and decision-making in factual verification tasks remains unclear. We ran an online study (N=68) manipulating three properties of LLM reasoning rationales: presentation format (instant vs. delayed vs. on-demand), correctness (correct vs. incorrect), and certainty framing (none vs. certain vs. uncertain). We found that correct rationales and certainty cues increased trust, decision confidence, and AI advice adoption, whereas uncertainty cues reduced them. Presentation format did not have a significant effect, suggesting users were less sensitive to how reasoning was revealed than to its reliability. Participants indicated they use rationales to primarily audit outputs and calibrate trust, where they expected rationales in stepwise, adaptive forms with certainty indicators. Our work shows that user-facing rationales, if poorly designed, can both support decision-making yet miscalibrate trust.

==> package.tex <==
% Remove the "review" option to generate the final version.
% \usepackage[review]{acl}

% Standard package includes
\usepackage{times}
\usepackage{latexsym}

% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
\usepackage[T1]{fontenc}
% For Vietnamese characters
% \usepackage[T5]{fontenc}
% See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% This assumes your files are encoded as UTF8
\usepackage[utf8]{inputenc}

% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
\usepackage{microtype}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}

% If the title and author information does not fit in the area allocated, uncomment the following
%
%\setlength\titlebox{<dim>}
%
% and set <dim> to something 5cm or larger.

% =========================================================================================

\usepackage{acronym}
\usepackage{enumitem} % Add this line


==> tables/survey_anova.tex <==

% \begin{table}[!htbp]
% \centering
% \footnotesize
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccc@{}}
% \toprule
% \textbf{Category} & \textbf{Variable} & \textbf{Effect Size} & \textbf{P-Value} & \textbf{Significance} \\ 
% \midrule
% \multirow{3}{*}{\textbf{Trust Info}}   
%                   & Strategy    & .618 & .539 & ns \\
%                   & Confidence Cue  & 4.778 & .009 & $**$ \\
%                   & Correctness & 4.552 & .034 & $*$ \\ 
% \hline

% \multirow{3}{*}{\textbf{Trust Meter}}    
%                   & Strategy    & 1.150 & .318 & ns \\
%                   & Confidence Cue  & 5.471 & .005 & $**$ \\
%                   & Correctness & 8.446 & .004 & $**$ \\ 

% \hline

% \multirow{3}{*}{\textbf{Trust System}} 
%                   & Strategy    & .313 & .731 & ns \\
%                   & Confidence Cue  & 3.097 & .021 & $*$ \\
%                   & Correctness & 4.552 & .125 & ns \\ 
% \hline

% \multirow{3}{*}{\textbf{Cognitive Load}}    
%                   & Strategy    & .786 & .456 & ns \\
%                   & Confidence Cue  & .167 & .846 & ns \\
%                   & Correctness & 2.194 & .139 & ns \\ 
% \hline

% \multirow{3}{*}{\textbf{Decision Confidence}}    
%                   & Strategy    & .327 & .721 & ns \\
%                   & Confidence Cue  & 6.524 & .002 & $**$ \\
%                   & Correctness & .283 & .595 & ns \\ 

% % \multirow{3}{*}{\textbf{Decision Performance}}    
% %                   & Strategy    & / & / & / \\ 
% %                   & Confidence Cue  & / & / & --- \\
% %                   & Correctness & --- & --- & --- \\ 

% \bottomrule
% \end{tabular*}

% \caption{Result of mix-ANOVA analysis.}
% \label{tab:survey_anova}
% \end{table}


\begin{table}[!htbp]
\centering
\footnotesize
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llccc@{}}
\toprule
\textbf{Category} & \textbf{Measure} & \textbf{Effect Size} & \textbf{P-Value} & \textbf{Significance} \\ 
\midrule
\multirow{4}{*}{\textbf{Strategy}}   
                  & Trust Info           & .618  & .539 & ns \\
                  & Trust System         & .313  & .731 & ns \\
                  & Trust Meter          & 1.150 & .318 & ns \\
                  % & Cognitive Load       & .786  & .456 & ns \\
                  & Decision Confidence  & .327  & .721 & ns \\ 
\hline
\multirow{4}{*}{\textbf{Confidence Cue}}    
                  & Trust Info           & 4.778 & .009 & $**$ \\
                  & Trust System         & 3.097 & .021 & $*$ \\
                  & Trust Meter          & 5.471 & .005 & $**$ \\
                  % & Cognitive Load       & .167  & .846 & ns \\
                  & Decision Confidence  & 6.524 & .002 & $**$ \\ 
\hline
\multirow{4}{*}{\textbf{Correctness}} 
                  & Trust Info           & 4.552 & .034 & $*$ \\
                  & Trust System         & 4.552 & .125 & ns \\
                  & Trust Meter          & 8.446 & .004 & $**$ \\
                  % & Cognitive Load       & 2.194 & .139 & ns \\
                  & Decision Confidence  & .283  & .595 & ns \\ 
\bottomrule
\end{tabular*}
\caption{Result of the mixed-ANOVA analysis.}
\vspace{-5.0mm}
\label{tab:survey_anova}
\end{table}
